Federated Stain Normalization for Computational Pathology

Although deep federated learning has received much attention in recent years, progress has been made mainly in the context of natural images and barely for computational pathology. However, deep federated learning is an opportunity to create datasets that reflect the data diversity of many laboratories. Further, the effort of dataset construction can be divided among many. Unfortunately, existing algorithms cannot be easily applied to computational pathology since previous work presupposes that data distributions of laboratories must be similar. This is an unlikely assumption, mainly since different laboratories have different staining styles. As a solution, we propose BottleGAN, a generative model that can computationally align the staining styles of many laboratories and can be trained in a privacy-preserving manner to foster federated learning in computational pathology. We construct a heterogenic multi-institutional dataset based on the PESO segmentation dataset and improve the IOU by 42\% compared to existing federated learning algorithms. An implementation of BottleGAN is available at https://github.com/MECLabTUDA/BottleGAN

==> sup.tex <==
The discriminators are trained to minimize
\begin{equation}

\begin{aligned}
    \mathcal{L}_{disc} = &\frac{1}{NM} \sum_{i=1}^{N} \sum_{j=1}^{M} D_s(G_s(c_j | e_{x_i}) | e_{x_i}) + \frac{1}{N} \sum_{i=1}^{N} D_c(
    G_{s^{-1}}(x_i | e_{x_i} )) \\ 
    & - \frac{1}{N} \sum_{i=1}^{N}  D_s(x_i |e_{x_i}) - \frac{1}{M} \sum_{i=j}^{M} D_c(c_j).
\end{aligned}
\end{equation}
The generators, in turn, are trained to minimize
\begin{equation}
\begin{aligned}
    \mathcal{L}_{gen} = & - \frac{1}{NM} \sum_{i=1}^{N} \sum_{j=1}^{M} D_s(G_s(c_j | e_{x_i}) | e_{x_i})   - \frac{1}{N} \sum_{i=1}^{N} D_c( G_{s^{-1}}(x_i | e_{x_i} )) \\
    & + \lambda_{cyc}   \mathcal{L}_{cyc} + \lambda_{idt}   \mathcal{L}_{idt},
\end{aligned}
\end{equation}
where $\mathcal{L}_{cyc}$ is defined as

\begin{equation}
    \mathcal{L}_{cyc} = \frac{1}{N} \sum_{i=1}^{N} ||G_s(G_{s^{-1}}(x_i | e_{x_i} ) | e_{x_i}), x_i||_1 + \frac{1}{NM} \sum_{i=1}^{N} \sum_{j=1}^{M}||G_{s^{-1}}(G_s(c_j | e_{x_i}) | e_{x_i}), c_j||_1
\end{equation}

and $\mathcal{L}_{idt}$ as 

\begin{equation}
    \mathcal{L}_{idt} = \frac{1}{NM} \sum_{i=1}^{N} \sum_{j=1}^{M} ||G_{s^{-1}}(c_j | e_{x_i}), c_j||_1 + \frac{1}{N} \sum_{i=1}^{N} ||G_s(x_i | e_{x_i}), x_i||_1.
\end{equation}

Described in words, the types of losses are identical to those of CycleGAN but reflect that $G_s$, $G_s^{-1}$, and $D_s$ can be conditioned on many staining styles. Further, the WassersteinGAN \cite{arjovsky2017wasserstein} adversarial loss is used for a more stable training behavior. Both losses $\mathcal{L}_{gen}$ and $\mathcal{L}_{disc}$ are iteratively minimized as it is typical for GANs. 

As a side note, we would like to justify our decision to train two generators instead of one. In theory, one generator, like in the StarGAN \cite{choi2018stargan} or StarGANv2 \cite{choi2020starganv2} frameworks, would be sufficient to represent both the staining style functions and the inverse ones. However, we identify a problem in the training algorithm. When running a cycle of BottleGAN and using only one generator, 50\% is either mapping to the reference staining style or mapping from the reference staining style. Consequently, all other staining styles must share the remaining 50\% influence on the gradients. If two generators are used, this imbalance does no longer exists.
